Spade: A Real-Time Fraud Detection Framework on Evolving Graphs (Complete Version)

Real-time fraud detection is a challenge for most financial and electronic commercial platforms. To identify fraudulent communities, Grab, one of the largest technology companies in Southeast Asia, forms a graph from a set of transactions and detects dense subgraphs arising from abnormally large numbers of connections among fraudsters. Existing dense subgraph detection approaches focus on static graphs without considering the fact that transaction graphs are highly dynamic. Moreover, detecting dense subgraphs from scratch with graph updates is time consuming and cannot meet the real-time requirement in industry. To address this problem, we introduce an incremental real-time fraud detection framework called Spade. Spade can detect fraudulent communities in hundreds of microseconds on million-scale graphs by incrementally maintaining dense subgraphs. Furthermore, Spade supports batch updates and edge grouping to reduce response latency. Lastly, Spade provides simple but expressive APIs for the design of evolving fraud detection semantics. Developers plug their customized suspiciousness functions into Spade which incrementalizes their semantics without recasting their algorithms. Extensive experiments show that Spade detects fraudulent communities in real time on million-scale graphs. Peeling algorithms incrementalized by Spade are up to a million times faster than the static version.

==> background.tex <==
%%%%%% Section 2 %%%%%%%
\section{Background}
\label{sec-pre}
\vspace{-0.3ex}

\begin{table}[tb!]
	\caption{Representative random walk}
  \label{tab:mf}
  \begin{scriptsize}
	  \begin{center}
		  \vspace{-5mm}
		  \setlength{\tabcolsep}{0.5em}
		  \begin{tabular}{|c|c|c|c|c|}
			\hline
			\multirow{2}{*}{} & \multirow{2}{*}{xxxx} & \multirow{2}{*}{xxx} & \multicolumn{2}{c|}{xxx} \\ \cline{4-5} 
								 &                       &                       & Exact index                 & Approximate index                 \\ \hline
		
								 XXX & 11   & 12 \cite{} & 13\cite{} & 14\cite{}\\ \hline
								 XXX & \cite{} & \cite{} & \cite{}  &  $-$ \\ \hline
								 XXX & \cite{} &  \cite{} & \cite{} & \cite{} \\ \hline
			\end{tabular}
	  \end{center}
  \end{scriptsize}
\end{table}


This  section  presents  the  background  for  the  technical discussions and then the problem statement. Some frequently used notations are summarized in Tab~\ref{tab-notations}. 


==> complexity.tex <==
\begin{table}[tb]
    %\setlength{\abovecaptionskip}{10pt}
    %\setlength{\belowcaptionskip}{10pt}
    %\captionsetup{font={scriptsize}}
    \caption{Complexity of existing algorithms (Before $2013$)}\label{tab:complexity1}
    \vspace{-3mm}
    \centering
    \begin{tabular}{|c|c|}
      \hline
      {\bf Algorithm} & {\bf Complexity}  \\
      \hline
      Ford–Fulkerson algorithm~\cite{ford1956maximal} & $O(|E||f_{max}|)$   \\
      \hline
      Push-relabeled algorithm~\cite{cherkassky1997implementing} & $O(|V|^2\sqrt{|E|})$   \\
      \hline
      Pseudoflow~\cite{hochbaum2008pseudoflow} & $O(|V|^2|E|)$   \\
      \hline
      Edmonds–Karp algorithm~\cite{edmonds1972theoretical} & $O(|V||E|^2)$   \\
      \hline
      Dinic's algorithm with dynamic trees~\cite{dinic1970algorithm}  & $O(|V|^2|E|)$   \\
      \hline
      James B Orlin's algorithm~\cite{orlin2013max} & $O(|V||E|)$    \\
      \hline
    \end{tabular}
    \end{table}

    \begin{table}[tb]
        %\setlength{\abovecaptionskip}{10pt}
        %\setlength{\belowcaptionskip}{10pt}
        %\captionsetup{font={scriptsize}}
        \caption{Complexity of existing algorithms (Between $2014$-$2020$)}\label{tab:complexity2}
        \vspace{-3mm}
        \centering
        \begin{tabular}{|c|c|}
          \hline
          {\bf Algorithm} & {\bf Complexity}  \\
          \hline
          Algo 1 &  \\
          \hline
        \end{tabular}
        \end{table}
        

==> tab-batchsize-backup.tex <==
\begin{table*}[tb]
\begin{footnotesize}
\begin{tabular}{|c|ccc||ccc|ccc|ccc|ccc|ccc|ccc|}
\hline 
                                  & \multicolumn{3}{c||}{Peeling algorithms (seconds)}                                                                  & \multicolumn{3}{c|}{ $|\Delta E| = 1$ ($us$)}                                                           & \multicolumn{3}{c|}{$|\Delta E| = 10$ ($us$)}                                                          & \multicolumn{3}{c|}{$|\Delta E| = 100$ ($us$)}                                                         & \multicolumn{3}{c|}{$|\Delta E| = 1K$ ($us$)}                                                        & \multicolumn{3}{c|}{$|\Delta E| = 10K$ ($us$)}                                                       & \multicolumn{3}{c|}{$|\Delta E| = 100K$ ($us$)}                                                      \\ \hline \hline
\textbf{Datasets} & \multicolumn{1}{c|}{$\DENG$} & \multicolumn{1}{c|}{$\DENGW$} & $\Fraudar$ & \multicolumn{1}{c|}{\IncDENG} & \multicolumn{1}{c|}{$\DENGW$} & $\Fraudar$ & \multicolumn{1}{c|}{\IncDENG} & \multicolumn{1}{c|}{$\DENGW$} & $\Fraudar$ & \multicolumn{1}{c|}{\IncDENG} & \multicolumn{1}{c|}{$\DENGW$} & $\Fraudar$ & \multicolumn{1}{c|}{\IncDENG} & \multicolumn{1}{c|}{$\DENGW$} & $\Fraudar$ & \multicolumn{1}{c|}{\IncDENG} & \multicolumn{1}{c|}{$\DENGW$} & $\Fraudar$ & \multicolumn{1}{c|}{\IncDENG} & \multicolumn{1}{c|}{$\DENGW$} & $\Fraudar$ \\ \hline
Grab1                             & \multicolumn{1}{c|}{$12$}               & \multicolumn{1}{c|}{$14$}               & $12$               & \multicolumn{1}{c|}{6517}               & \multicolumn{1}{c|}{17469}              & 6                  & \multicolumn{1}{c|}{3117}               & \multicolumn{1}{c|}{11613}              & 6                  & \multicolumn{1}{c|}{519}                & \multicolumn{1}{c|}{1983}               & 6                  & \multicolumn{1}{c|}{108}                & \multicolumn{1}{c|}{281}                & 6                  & \multicolumn{1}{c|}{25}                 & \multicolumn{1}{c|}{55}                 & 4                  & \multicolumn{1}{c|}{5}                  & \multicolumn{1}{c|}{10}                 & 1                  \\ \hline
Grab2                             & \multicolumn{1}{c|}{17}                 & \multicolumn{1}{c|}{20}                 & 16                 & \multicolumn{1}{c|}{6604}               & \multicolumn{1}{c|}{18413}              & 8                  & \multicolumn{1}{c|}{3484}               & \multicolumn{1}{c|}{11280}              & 8                  & \multicolumn{1}{c|}{634}                & \multicolumn{1}{c|}{1782}               & 8                  & \multicolumn{1}{c|}{138}                & \multicolumn{1}{c|}{249}                & 8                  & \multicolumn{1}{c|}{33}                 & \multicolumn{1}{c|}{45}                 & 6                  & \multicolumn{1}{c|}{7}                  & \multicolumn{1}{c|}{8}                  & 2                  \\ \hline
Grab3                             & \multicolumn{1}{c|}{23}                 & \multicolumn{1}{c|}{27}                 & 22                 & \multicolumn{1}{c|}{6716}               & \multicolumn{1}{c|}{18862}              & 11                 & \multicolumn{1}{c|}{3864}               & \multicolumn{1}{c|}{10892}              & 11                 & \multicolumn{1}{c|}{750}                & \multicolumn{1}{c|}{1560}               & 10                 & \multicolumn{1}{c|}{186}                & \multicolumn{1}{c|}{211}                & 10                 & \multicolumn{1}{c|}{44}                 & \multicolumn{1}{c|}{38}                 & 8                  & \multicolumn{1}{c|}{8}                  & \multicolumn{1}{c|}{7}                  & 2                  \\ \hline
Grab4                             & \multicolumn{1}{c|}{27}                 & \multicolumn{1}{c|}{28}                 & 28                 & \multicolumn{1}{c|}{6562}               & \multicolumn{1}{c|}{17469}              & 14                 & \multicolumn{1}{c|}{4108}               & \multicolumn{1}{c|}{11661}              & 12                 & \multicolumn{1}{c|}{878}                & \multicolumn{1}{c|}{1970}               & 13                 & \multicolumn{1}{c|}{206}                & \multicolumn{1}{c|}{267}                & 12                 & \multicolumn{1}{c|}{51}                 & \multicolumn{1}{c|}{50}                 & 9                  & \multicolumn{1}{c|}{10}                 & \multicolumn{1}{c|}{9}                  & 3                  \\ \hline
Amazon                            & \multicolumn{1}{c|}{0.49}               & \multicolumn{1}{c|}{0.53}               & 0.43               & \multicolumn{1}{c|}{350}                & \multicolumn{1}{c|}{342}                & 1                  & \multicolumn{1}{c|}{186}                & \multicolumn{1}{c|}{191}                & -                  & \multicolumn{1}{c|}{29}                 & \multicolumn{1}{c|}{30}                 & -                  & \multicolumn{1}{c|}{7}                  & \multicolumn{1}{c|}{6}                  & -                  & \multicolumn{1}{c|}{-}                  & \multicolumn{1}{c|}{-}                  & -                  & \multicolumn{1}{c|}{-}                  & \multicolumn{1}{c|}{-}                  & -                  \\ \hline
Wiki-Vote                         & \multicolumn{1}{c|}{0.022}              & \multicolumn{1}{c|}{0.021}              & 0.017              & \multicolumn{1}{c|}{184}                & \multicolumn{1}{c|}{149}                & 2                  & \multicolumn{1}{c|}{98}                 & \multicolumn{1}{c|}{84}                 & 1                  & \multicolumn{1}{c|}{29}                 & \multicolumn{1}{c|}{28}                 & 1                  & \multicolumn{1}{c|}{5}                  & \multicolumn{1}{c|}{5}                  & -                  & \multicolumn{1}{c|}{1}                  & \multicolumn{1}{c|}{1}                  & -                  & \multicolumn{1}{c|}{-}                  & \multicolumn{1}{c|}{-}                  & -                  \\ \hline
Epinion                           & \multicolumn{1}{c|}{0.25}               & \multicolumn{1}{c|}{0.26}               & 0.23               & \multicolumn{1}{c|}{170}                & \multicolumn{1}{c|}{151}                & 5                  & \multicolumn{1}{c|}{83}                 & \multicolumn{1}{c|}{80}                 & 3                  & \multicolumn{1}{c|}{32}                 & \multicolumn{1}{c|}{30}                 & 2                  & \multicolumn{1}{c|}{10}                 & \multicolumn{1}{c|}{10}                 & 2                  & \multicolumn{1}{c|}{3}                  & \multicolumn{1}{c|}{3}                  & 1                  & \multicolumn{1}{c|}{1}                  & \multicolumn{1}{c|}{1}                  & -                  \\ \hline
\end{tabular}
\end{footnotesize}
\caption{Time taken for incremental maintenance with \Spade{} by varying batch sizes (avg. time for one edge, - means $ < 1us$)}\label{tab:batchsize}
\end{table*}
